ReLyMe: Improving Lyric-to-Melody Generation by Incorporating Lyric-Melody Relationships

Lyric-to-melody generation, which generates melody according to given lyrics, is one of the most important automatic music composition tasks. With the rapid development of deep learning, previous works address this task with end-to-end neural network models. However, deep learning models cannot well capture the strict but subtle relationships between lyrics and melodies, which compromises the harmony between lyrics and generated melodies. In this paper, we propose ReLyMe, a method that incorporates Relationships between Lyrics and Melodies from music theory to ensure the harmony between lyrics and melodies. Specifically, we first introduce several principles that lyrics and melodies should follow in terms of tone, rhythm, and structure relationships. These principles are then integrated into neural network lyric-to-melody models by adding corresponding constraints during the decoding process to improve the harmony between lyrics and melodies. We use a series of objective and subjective metrics to evaluate the generated melodies. Experiments on both English and Chinese song datasets show the effectiveness of ReLyMe, demonstrating the superiority of incorporating lyric-melody relationships from the music domain into neural lyric-to-melody generation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> content/sections/3-principles.tex <==
\section{Method}
% In this section, we first introduce the principles of lyric-melody relationships, then we describe the constrained decoding mechanism in \myname{} and the corresponding reward formulation, at last, we show the pipelines when applying \myname{} to different lyric-to-melody generation systems.
% \subsection{Principles}
% \label{sec:preliminary}
% The lyric-melody relationships mean the combining relationships between the rules of lyrics and the rules of the melodies within the scope of unified content, which control the interplay between the lyrics and the melodies. According to~\cite{yu2008study} which described the lyric-melody relationships of traditional Chinese folk music from the view of composer or musicians, these combining relationships are reflected in tone, rhythm, and structure. We follow these three aspects and extend them to different types of languages (tonal language like Mandarin, ``stress accent'' languages like English). An example shows the principles we discuss below can be found in Figure~\ref{fig:case}.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{content/figs/case.pdf}
%     \caption{The music sheet of a Mandarin song ``Rainbow'' by Jay Chou. The colorful boxes illustrate the lyric-melody relationships we formulate.}
%     \label{fig:case}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\textwidth]{content/figs/pitch shape.pdf}
%     \caption{The pitch shape of four main tones in Mandarin.}
%     \label{fig:tones}
% \end{figure}

% \begin{figure}[tbp]
% 	\centering
% 	\subfloat[A bad case that breaks pitch shape principle. The word ``d\.i f\=ang'' of the lyrics means ``place'', but it sounds like ``d\'{i} f\=ang'', which means ``enemy''.]{\label{fig:case_pitch_shape}\includegraphics[width=0.5\textwidth,trim={0cm, 0cm, 0cm, 1.4cm},clip=true]{content/figs/principle_case0.pdf}}\\
% 	\subfloat[A bad case that breaks pitch transition principle. The ``d\=eng t\v{a}'' of the lyrics means ``lighthouse'', but it sounds like ``d\v{e}ng t\=a'', which means ``waiting for him''.]{\label{fig:case_pitch_transition}\includegraphics[width=0.5\textwidth]{content/figs/principle_case1.pdf}}\\
% 	\caption{Bad cases of pitch principles.}
% \end{figure}

% \begin{figure*}[!thb]
%     \centering
%     \includegraphics[width=0.8\textwidth]{content/figs/pitch transition.pdf}
%     \caption{The harmony degrees (excellent, good, fair, bad) of the pitch difference between neighboring notes given each adjacent tone pair in Mandarin.}
%     \label{fig:pitch_transition}
% \end{figure*}

\subsubsection{Tone} 
\
\newline
When the lyrics are sung with given melody, the pitch of the lyrics is determined by the melody instead of the intrinsic tone or stress~\cite{zhang2021pdaugment}. Aligning the pitch of the melody with the original pitch of the lyrics is essential for reducing semantic misunderstandings when performing songs~\cite{yu2008study,guo2021automatic}.

About 60\% of languages have tone~\footnote{https://en.wikipedia.org/wiki/Tone\_(linguistics)} (called tonal language)~\cite{yip2002tone}, such as Chinese, Vietnamese, Thai.
Tone is the pitch information in tonal languages that helps distinguish words with the spelling but different meanings. In most tonal languages, a single tone is assigned to a syllable.
In order to align the melodies with the lyrics at the tonal level, we consider the following three granularities of lyric-melody relationships:

\begin{itemize}
    \item \textbf{Pitch shape of a single tone.} For each syllable in lyrics, when it corresponds to more than one notes in the melody, the predefined shape of the tone should coincide with the pitch flow of the corresponding note group. Take Mandarin as an example, which contains four main tones (high level tone, rising tone, falling-rising tone, falling tone, denoted as tone1, tone2, tone3 and tone4) and a light tone (unstressed syllable pronounced without its original pitch in Chinese pronunciation, denoted tone5)~\cite{hu2017sungwords}. The predefined shapes of four main tones are shown as Figure~\ref{fig:tones} and an example that breaks this principle can be found in Figure~\ref{fig:case_pitch_shape}.
    \item \textbf{Pitch transition between adjacent tones.} For a pair of adjacent syllables within the same sentence, the pitch flow of the corresponding adjacent notes needs to be in line with the pitch transition between tones, otherwise may leads to the misunderstanding like Figure~\ref{fig:case_pitch_transition}. According to the practice in natural speech, we measure the degree of harmony (excellent, good, fair, poor) for the pitch difference between neighboring notes given each adjacent tone pair,
    as shown in Figure~\ref{fig:pitch_transition}.
    \item \textbf{Pitch contour of a whole sentence.} Lyrics, as a form of text, have their inherent intonation for each sentence to express different emotions and meanings. The pitch contour of a whole sentence depends on the corresponding melody, so the pitch direction of the melody needs to be matched to the inherent intonation of the sentence to ensure that correct meaning is conveyed. For example, an interrogative tends to align with a rising melody (see the orange box of Figure~\ref{fig:case}).
\end{itemize}

For tonal languages, the pitch of the melody is aligned with the tone of the lyrics and all of above three granularities are considered. While for ``stress accent'' languages such as English, which do not have tones, we only consider the pitch contour relationship.

\begin{figure}[tbp]
	\centering
	\subfloat[A bad case that assigns an auxiliary word to downbeat. The question auxiliary ``ma'' is heard as ``m\=a'', which means mother.]{\label{fig:case_strong_weak}\includegraphics[width=0.5\textwidth,trim={0cm, 0cm, 0cm, 1.2cm},clip=true]{content/figs/principle_case3.pdf}}\\
	\subfloat[A bad case that breaks the principle of pause positions. There is a pause caused by long notes inside a word (red arrow), while an appropriate pause should be at the blue arrow. This mismatch may spoil the coherence of the song.]{\label{fig:case_pause}\includegraphics[width=0.5\textwidth]{content/figs/principle_case2.pdf}}\\
	\caption{Bad cases of rhythm principles.}
\end{figure}

\subsubsection{Rhythm}
We consider the rhythmic relationship in two dimensions: 1) intensity at a certain moment, reflected in strong and weak positions; 2) temporal alignment, reflected in pause positions.
\begin{itemize}
    \item \textbf{Strong and Weak Positions.} Both melodies and lyrics have the "strong" and "weak" elements, and the movement marked by the regulated succession of these elements is described as rhythm. A songwriter might align downbeats or accents with stressed syllables or important words~\footnote{https://en.wikipedia.org/wiki/Prosody\_(music)}. Aligning the rhythm of melody and lyrics helps convey meaning, express empathy and render emotion. The strong and weak positions in melody lines could be determined by multiple factors~\cite{yu2008study}: pitch, duration, syncopation, meter, and so on. During automatic melody generation, for simplicity, the strong and weak beats can be derived from the predefined time signature~\cite{benward2003introduction}. In lyrics, the strong and weak positions are mainly influenced by oral speaking habits, specific semantics, intent of speakers, and expressed emotions. For example, in spoken language, the auxiliary words tend to be pronounced lightly, while the keywords in the lyrics are often regarded as accents, which are pronounced louder to attract the attention of listeners and emphasize the elements. The strong and weak positions of melodies are aligned with those of lyrics to ensure harmony of performance and correct meaning. Specifically, the keywords often correspond to the strong positions of the melody while auxiliary words should be placed on the weak positions.
    \item \textbf{Pause Positions.} Pauses in speech divide the entire sentence into several parts with separate meanings (called prosodic phrases) to help the listener understand. Sentences with the same content but different pause positions can have completely different meanings, and the division of prosodic phrases that defies common sense can lead to confusion for listeners. In melody, the pauses are caused by either~\textit{REST} notes~\footnote{https://en.wikipedia.org/wiki/Rest\_(music)} or long notes and split the melody into musical phrases, which make complete musical sense when heard on their own. When the lyrics are sung with given melodies, the pause positions are no longer influenced by the spoken idiom but are controlled by the pauses in the melody. When syllables of the same prosodic phrase are assigned to different musical phrases, a phenomenon called ``broken phrases'' occurs, which impairs the harmony between the melody and the lyrics and makes the lyrics hard to understand for listeners. Thus, inappropriate \textit{REST} notes or long notes can be detrimental to the music. We summarize the following cases which lead to the dissonance and misunderstanding (examples can be found in Figure~\ref{fig:case_pause}): 1) \textit{REST} notes are located inside the prosodic phrase; 2) long notes are assigned to non-final syllables of a prosodic phrase; 3) there are neither \textit{REST} notes nor long notes at the end of the sentence.
\end{itemize}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{content/figs/principle_case2.pdf}
%     \caption{A bad case that breaks the principle of pause positions. There is a pause caused by long notes inside a word (red arrow), while an appropriate pause should be at the blue arrow. This mismatch may spoil the coherence of the song.}
%     \label{fig:case_pause}
% \end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{content/figs/principle_case4.pdf}
    \caption{An example that shows the structure relationships between lyrics and melody.}
    \label{fig:case_structure}
\end{figure}

\subsubsection{Structure}
\
\newline
At the full song level, the structure of lyrics and melody are constrained and influenced by each other.
In music, \textit{form}\footnote{https://en.wikipedia.org/wiki/Musical\_form} refers to the structure of a musical composition or performance, including repetition, transition and development~\cite{zhang2021structure}. 
To better convey emotion and show artistry, lyrics and melody which belong to the same musical form would share the same characteristics like rhyme or motives. Specifically, in lyric-to-melody generation, the melody segments that correspond to the lyrics of the same structure tend to have similar pitch flows (see Figure~\ref{fig:case_structure}).

==> content/sections/4-methods.tex <==
% \section{Method}
% In this section, we first outline our \myname{}, then we describe detailed designs of constrained decoding in our \myname{}, and finally, we give specific definitions of the constraint scores in Mandarin.
% \subsection{Pipeline Overview}
% Our \myname{} is a method which integrates the principles of music theory into the lyric-to-melody generation process, in order to enhance the harmony between the composed melody and the given lyrics. \myname{} can be applied to different lyric-to-melody generation systems, and in this work, we apply \myname{} in two systems: 1) TeleMelody~\cite{ju2021telemelody}, a two-stage lyric-to-melody generation system with musical template; and 2) SongMASS~\cite{sheng2021songmass}, an end-to-end lyric-to-melody generation system with pretraining process.
% TeleMelody consists of a lyric-to-template module and template-to-melody module, using the template as the bridge to narrow the gap between lyric and melody, as well as improving the generation controllability by adjusting the template during the generating process. According to music theory described in Section~\ref{sec:preliminary}, \myname{} adjust both the lyric-to-template module and template-to-melody module, guide them to generate templates or melodies which obey the principles.
% SongMASS pretrains an end-to-end model to generate melody from the given lyrics directly, and \myname{} integrates those musical principles during the inference process.
% \myname{} incorporates the relationships between lyrics and melody into aforementioned lyric-to-melody generation system by constrained decoding mechanism, which will be introduced as follow.
% % \myname{} formulates the music theory and contains two schemes: combined score selection and constrained decoding, which will be introduced as follow. 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\textwidth,trim={2cm, 21.5cm, 11cm, 3.5cm},clip=true]{content/figs/constrained_decoding.pdf}
%     \caption{The inference process of constrained decoding. The constraints are integrated at each inference step (as gray arrows).}
%     \label{fig:constrained_decoding}
% \end{figure}


\subsection{Constrained Decoding}
Considering that the generation process of most of current neural network lyric-to-melody generation systems is auto-regressive, \myname{} adds constraints that derived from above principles at each decoding step. Specifically, during inference, adjusting the probabilities of each decoding step can influence the current generated token, which further affects the subsequent tokens.
% As shown in Figure~\ref{fig:constrained_decoding}, following the idea of \cite{guo2021automatic}, w
% We impose the constraints in the decoding phase. 

Denote the training lyric-melody pair as $\{(\bm{x}, \bm{y}) \in (\bm{\mathcal{X}}, \bm{\mathcal{Y}})\}$. 
The original score function of beam search in generation system at ith decoding step is:
\begin{equation}
\begin{aligned}
    s_i = logP(y_i|y_{0:i-1}, x).
\end{aligned}
\end{equation}
At each decoding step, the constrained decoding mechanism adds the reward $R_{cons}$ directly to the score.
$R_{cons}(y_{0:i}, x)$ denotes the total reward at ith decoding step under the musical constraints, which consists of three parts: 1) the tone reward $R_t(y_{0:i}, x)$, 2) the rhythm reward $R_r(y_{0:i}, x)$, and 3) the structure reward $R_s(y_{0:i}, x)$. The formulation of these three rewards are defined below.
Thus, the score function in constrained decoding mechanism can be described as:
\begin{equation}
    s'_i = logP(y_i|y_{0:i-1}, x) + R_{cons}(y_{0:i}, x).
\end{equation}
Then $s'_i$ is used in beam search as the new score function.


\subsection{Reward Formulation based on Musical Principles}
\label{sec:formulation}
In this part, we give the formulation for three rewards based on the principles of lyric-melody relationships, which  will be used in aforementioned constrained decoding mechanism.
For a lyric sequence $\bm{x}$, the corresponding syllable sequence is $\bm{s} = \{s_1, ..., s_n\}$, and the tone sequence is described as $\bm{t} = \{t_1, ..., t_n\}$. 
% Each note in melody $\bm{y}$ is matched with one syllable.
The melody $\bm{y}$ consists of a sequence of notes $\bm{n} = \{n_1, ..., n_m\} (n \leq m)$ and one syllable can be matched with one note or multiple notes.
% one note is matched with one syllable (i.e. $n_i$ is corresponding to $s_i$). 
Here, we formulate the rewards derived from the relationships between lyrics and melodies (in Section~\ref{sec:preliminary}) as follows:
\subsubsection{Rewards of Tone}
\
\newline
The pitch sequence corresponding to note sequence is $\bm{p} = \{p_1, ..., p_n\}$. The total tone reward $R_t(y_{0:i}, x)$ is the sum of the following three rewards.
\begin{itemize}
    \item \textbf{Pitch Shape Reward.} 
    This reward is only considered when more than one notes $\{n_j, ..., n_{j+l}\}$ are assigned to a syllable $s_i$.
    Each tone of a syllable in tonal languages has its intrinsic pitch shape, when the pitch shape of the single tone is matched with that of corresponding notes, we assign the reward $R_{ps}(t_{i}, p_{j:j+l}) = 1$, otherwise the reward is 0.
    \item \textbf{Pitch Transition Reward.} 
    Given each adjacent tone pair $\{t_{i-1}, t_i\}$ in tonal languages, the pitch difference between the corresponding adjacent notes $\{n_{j-1}, n_j\}$ will be classified into different harmony degrees (excellent, good, fair, bad) according to linguists and musicians (such as Mandarin in Figure~\ref{fig:pitch_transition}). We assign a reward $R_{pt}(t_{i-1:i}, p_{j-1:j})$ to current decoding step $i$ based on the harmony degree of the pitch difference $\Delta p_j = p_j - p_{j-1}$ given the corresponding tone pair $(t_{i-1}, t_i)$. In practice, we assign the reward of 4.0, 3.5, 2.5, 0 when $\Delta p_j$ belongs to the harmony degree of excellent, good, fair, and bad respectively. 
    \item \textbf{Pitch Contour Reward.} 
    Assume that $\{t_{i-l}, ..., t_{i}\}$ is the tone sequence of a sentence, we calculate the reward of pitch contour $R_{pc}(t_{i-l:i}, x)$ according to the inherent intonation of the sentence and the pitch contour of corresponding melody. That is to say, when the inherent intonation and the pitch contour are both rising or falling, the reward is set to be 1, otherwise is 0.
\end{itemize}

\subsubsection{Rewards of Rhythm}
\
\newline
The beat sequence corresponding to note sequence is $\bm{b} = \{b_1, ..., b_n\}$. The total rhythm reward $R_r(y_{0:i}, x)$ is the sum of the following two rewards.
\begin{itemize}
    \item \textbf{W/S Position Reward.} When the strong or weak positions of lyrics and melody match, $R_{ws}(x_i, b_i)$ is assigned to 1, otherwise 0.
    \item \textbf{Pause Position Reward.} By word segmentation, we can obtain the positions that split words and sentences. The pause positions in melodies need to occur at those ``split'' positions, or phrases will be broken. Besides, there tends to be a corresponding pause in melody if this position splits two sentences. Thus, the reward $R_{ps}(x_i, b_i) = 0$ when the pause is not at a ``split'' position or there is no pause in melody between two sentences and $R_{ps}(x_i, b_i) = 1$ otherwise.
\end{itemize}
    
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.3\textwidth,trim={7.5cm, 13.7cm, 7cm, 9.9cm},clip=true]{content/figs/structure_matrix_big.pdf}
    \caption{An example of structure matrix $M_{struct}$, which means $\{n_1, n_2, n_3\}$, $\{n_6, n_7, n_8\}$, $\{n_{11}, n_{12}, n_{13}\}$ are of the same structure.}
    \label{fig:structure_matrix}
\end{figure}

\subsubsection{Reward of Structure}
\
\newline
    After the lyrics structure analysis, we can obtain a matrix $M_{struct}$ which indicates the structure of the lyrics. $M_{struct}^{ij} = 1$ if note i and note j are at the corresponding positions in the phrases of the same structure and $M_{struct}^{ij} = 0$ otherwise. An example of $M_{struct}$ can be seen in Figure~\ref{fig:structure_matrix}.
    
    Thus, we assign the structure reward $R_s(p_{0:i}, M_{struct}) = 2$ if the pitch of ith note $p_i$ is equal to the pitch of jth node $p_j$ (where i and j satisfy $M_{struct}^{ij} = 1$ and $j<i$) and assign $R_s = 1$ if the pitch difference between ith note and jth note is a multiple of 12. Otherwise, the structure reward is 0.


\subsection{Applications in Different Lyric-to-Melody Generation Systems}
\myname{} can be applied to different lyric-to-melody generation systems, and in this work, we apply \myname{} in two systems: 1) TeleMelody~\cite{ju2021telemelody}, a two-stage lyric-to-melody generation system with musical template; and 2) SongMASS~\cite{sheng2021songmass}, an end-to-end lyric-to-melody generation system with pretraining process. These two are the state-of-the-art systems in end-to-end and multi-stage lyric-to-melody generation systems respectively.

\noindent{\textbf{For TeleMelody.}}
TeleMelody consists of a lyric-to-template module and template-to-melody module, using the template as the bridge to narrow the gap between lyric and melody, as well as improving the generation controllability by adjusting the template during the generating process. \myname{} adjust both the lyric-to-template module and template-to-melody module, guide them to generate templates or melodies which obey the principles.
During the lyric-to-template module, we adjust the score of each step in beam search with the rhythmic constraints:
\begin{equation}
\begin{aligned}
    logP_{l2t}(\bm{z}|\bm{x}) = \sum_{i=0}^n[logP_{l2t}(z_i|z_{i-1:0},\bm{x}) \\
    + \lambda_r R_r(y_{0:i}, x)],
\end{aligned}
\end{equation}
where $z$ represents the output template of lyric-to-template module, $R_r(y_{0:i}, x)$ is the total rhythm reward of the ith decoding step and $\lambda_r$ represents a hyper-parameter that controls the influence of rhythmic constraint.
Meanwhile, the relationships of tone and structure are added in template-to-melody module:
\begin{equation}
\begin{aligned}
    logP_{t2m}(\bm{y}|\bm{z},\bm{x}) = \sum_{i=0}^n[logP_{t2m}(y_i|y_{i-1:0},\bm{z},\bm{x}) \\
    + \lambda_t R_t(y_{0:i}, x) + \lambda_s R_s(y_{0:i}, x)].
\end{aligned}
\end{equation}
$R_t(y_{0:i}, x)$ and $R_s(y_{0:i}, x)$ are the tone reward and structure reward of the ith step and $\lambda_t$ and $\lambda_s$ refer to hyper-parameters of constraints of tone and structure respectively.

\noindent{\textbf{For SongMASS.}}
SongMASS pretrains an end-to-end model to generate melody from the given lyrics directly, so the constraints of all three aspects are incorporated to decoding process at once:
\begin{equation}
    \begin{aligned}
    logP(\bm{y}|\bm{x}) = \sum_{i=0}^n[logP_{l2m}(y_i|y_{i-1:0}, \bm{x}) \\
    + \lambda_t R_t(y_{0:i}, x) + \lambda_r R_r(y_{0:i}, x) + \lambda_s R_s(y_{0:i}, x)].
    \end{aligned}
\end{equation}


